Residual-Christoffel Sampling for Random Feature Collocation of Linear PDEs

Random feature collocation fixes a randomly generated trial space and determines its coefficients from a linear least-squares system. Stability then depends on whether the sampled residual equations represent the geometry induced by the differential operator. We construct an operator-aware discretization in which the operator-applied features determine both the collocation measure and a coefficient whitening map. The randomized scheme combines a residual-Christoffel density with inverse-density weights, while a deterministic scalar-row alternative maximizes successive regularized log-determinant increments. Conditional on the realized trial space, the sampled whitened interior Gram is a spectral approximation to the reference Gram on the retained residual space, with sample complexity linear in the retained dimension up to a logarithmic factor. For uniformly analytic residual kernels, the associated operator has stretched-exponentially decaying eigenvalues and ridge effective dimension that is polylogarithmic in the inverse ridge scale. Experiments on scalar and vector equations, varied geometries, and one to three spatial dimensions show that residual-space sampling and whitening produce numerically full-rank transformed systems with substantially smaller condition numbers and iteration counts. The deterministic construction attains the lowest errors at the smallest scalar sample sizes. Residual-space geometry therefore yields a principled design for stable strong-form random feature collocation.

==> algorithms.tex <==
\makeatletter
\newcounter{algline}
\newcommand{\algorithmruletitle}[2]{%
  \refstepcounter{algorithm}%
  \def\@currentlabelname{#1}%
  \label{#2}%
  \par\noindent\rule{\textwidth}{0.55pt}\par
  \noindent\textbf{Algorithm~\thealgorithm} #1\par
  \noindent\rule{\textwidth}{0.35pt}\par
}
\newenvironment{algorithmlines}{%
  \begin{list}{\arabic{algline}:}{%
    \usecounter{algline}%
    \setlength{\leftmargin}{1.7em}%
    \setlength{\labelwidth}{1.25em}%
    \setlength{\labelsep}{0.25em}%
    \setlength{\itemindent}{0pt}%
    \setlength{\itemsep}{1.5pt}%
    \setlength{\parsep}{0pt}%
    \setlength{\topsep}{2pt}%
  }%
  \raggedright
}{\end{list}}
\makeatother

